OSS-Net: Memory Efficient High Resolution Semantic Segmentation of 3D Medical Data

Convolutional neural networks (CNNs) are the current state-of-the-art meta-algorithm for volumetric segmentation of medical data, for example, to localize COVID-19 infected tissue on computer tomography scans or the detection of tumour volumes in magnetic resonance imaging. A key limitation of 3D CNNs on voxelised data is that the memory consumption grows cubically with the training data resolution. Occupancy networks (O-Nets) are an alternative for which the data is represented continuously in a function space and 3D shapes are learned as a continuous decision boundary. While O-Nets are significantly more memory efficient than 3D CNNs, they are limited to simple shapes, are relatively slow at inference, and have not yet been adapted for 3D semantic segmentation of medical data. Here, we propose Occupancy Networks for Semantic Segmentation (OSS-Nets) to accurately and memory-efficiently segment 3D medical data. We build upon the original O-Net with modifications for increased expressiveness leading to improved segmentation performance comparable to 3D CNNs, as well as modifications for faster inference. We leverage local observations to represent complex shapes and prior encoder predictions to expedite inference. We showcase OSS-Net's performance on 3D brain tumour and liver segmentation against a function space baseline (O-Net), a performance baseline (3D residual U-Net), and an efficiency baseline (2D residual U-Net). OSS-Net yields segmentation results similar to the performance baseline and superior to the function space and efficiency baselines. In terms of memory efficiency, OSS-Net consumes comparable amounts of memory as the function space baseline, somewhat more memory than the efficiency baseline and significantly less than the performance baseline. As such, OSS-Net enables memory-efficient and accurate 3D semantic segmentation that can scale to high resolutions.

==> table_final/inference_results.tex <==
\begin{tabular}{>{\raggedright\arraybackslash}p{0.239\columnwidth}>{\centering\arraybackslash}p{0.21\columnwidth}>{\centering\arraybackslash}p{0.21\columnwidth}>{\centering\arraybackslash}p{0.21\columnwidth}}
    \hline
	Inference method & Relative voxelwise disagreement & Average runtime $2^{14}$ locations & Average runtime $2^{17}$ locations \\
	\hline
	Standard \cite{mescheder2019} & \multirow{2}{*}{$5.9658\cdot 10^{-6}$} & $5.3619\si{\second}$ & $5.3215\si{\second}$ \\
	Optimized &  & $2.6248\si{\second}$ & $2.6056\si{\second}$ \\
	\hline
\end{tabular}
